FlipTracker: Understanding Natural Error Resilience in HPC Applications

As high-performance computing systems scale in size and computational power, the danger of silent errors, i.e., errors that can bypass hardware detection mechanisms and impact application state, grows dramatically. Consequently, applications running on HPC systems need to exhibit resilience to such errors. Previous work has found that, for certain codes, this resilience can come for free, i.e., some applications are naturally resilient, but few studies have shown the code patterns---combinations or sequences of computations---that make an application naturally resilient. In this paper, we present FlipTracker, a framework designed to extract these patterns using fine-grained tracking of error propagation and resilience properties, and we use it to present a set of computation patterns that are responsible for making representative HPC applications naturally resilient to errors. This not only enables a deeper understanding of resilience properties of these codes, but also can guide future application designs towards patterns with natural resilience.

==> abstract.tex <==
\begin{abstract}
As high-performance computing systems scale in size and computational power,
the danger of silent errors,
%An important need for 
%extreme-scale HPC 
%simulations running on them need to more and more consider
%resilience 
%is to provide
%resilience 
%to silent errors, 
i.e., errors that can bypass hardware
detection mechanisms and impact application state, {\color{black} grows} dramatically.
Consequently, applications running on {\color{black} HPC} systems need to
exhibit resilience to such errors. Previous work has found
that, for certain codes, this resilience can come for
free, i.e., some applications are naturally resilient, but
%
%Although previous research has shown that a number of scientific 
%applications are naturally resilient, 
%However,
few studies 
have shown the code patterns---combinations or sequences of 
computations---that make an application naturally resilient.
%or a subset of it, naturally resilient. 
%fault tolerant
%MS: we should stick to either resilient or fault tolerant
%The latter is needed, though, to fully understand this property and to use it to explicitly create, naturally resilient applications. 
In this paper, we present \name, a framework designed to 
extract these patterns using fine-grained tracking of error propagation and 
%of error tolerance, 
resilience properties, and we use it to present a set of computation patterns that 
are responsible for making representative HPC applications 
naturally resilient to errors. 
This not only 
enables a deeper understanding of resilience properties of 
these codes, but also can guide future application designs towards  patterns with natural resilience. 
%%\color{red}{az: removed!}
%, but also helps guide future applications 
%design towards natural resilience.
%In our study,
%using a range of representative HPC programs,  we discover a set of resilient computation patterns.
%{\color{red} 
%we found that  resilient computation patterns can be summarized into six classes (AZ: seems not accurate)}

%MS: I took this out for new, since it seems like a very anticlimactic ending of an abstract - feel free to disagree
%We demonstrate, using a large fault injection campaign, that code regions in one 
%application can have different levels of resilience, depending on 
%the occurrence of any of these patterns and on the location of the error.
\end{abstract}
